Transcending Forgery Specificity with Latent Space Augmentation for Generalizable Deepfake Detection

Deepfake detection faces a critical generalization hurdle, with performance deteriorating when there is a mismatch between the distributions of training and testing data. A broadly received explanation is the tendency of these detectors to be overfitted to forgery-specific artifacts, rather than learning features that are widely applicable across various forgeries. To address this issue, we propose a simple yet effective detector called LSDA (\underline{L}atent \underline{S}pace \underline{D}ata \underline{A}ugmentation), which is based on a heuristic idea: representations with a wider variety of forgeries should be able to learn a more generalizable decision boundary, thereby mitigating the overfitting of method-specific features (see Fig.~\ref{fig:toy}). Following this idea, we propose to enlarge the forgery space by constructing and simulating variations within and across forgery features in the latent space. This approach encompasses the acquisition of enriched, domain-specific features and the facilitation of smoother transitions between different forgery types, effectively bridging domain gaps. Our approach culminates in refining a binary classifier that leverages the distilled knowledge from the enhanced features, striving for a generalizable deepfake detector. Comprehensive experiments show that our proposed method is surprisingly effective and transcends state-of-the-art detectors across several widely used benchmarks.

==> tables/cross-dataset.tex <==
\begin{table*}
\centering
\scalebox{0.70}{
\begin{tabular}
{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
\toprule
\multirow{2}*{Method}& \multicolumn{3}{c|}{FF-ALL} & \multicolumn{3}{c|}{FF-wo-DF} & \multicolumn{3}{c|}{FF-wo-F2F} & \multicolumn{3}{c|}{FF-wo-FS} & \multicolumn{3}{c|}{FF-wo-NT} & \multirow{2}*{Avg.}\\
\cline{2-16}
& \small{DFDC} & \small{CelebDF} & \small{DFD} & \small{DFDC} & \small{CelebDF} &\small{DFD} & \small{DFDC} & \small{CelebDF} &\small{DFD} & 
\small{DFDC} & \small{CelebDF} &\small{DFD} & \small{DFDC} &\small{CelebDF} &\small{DFD}  \\ 
\midrule
Xception~\cite{rossler2019faceforensics++} &0.651 &0.672 &0.727 &0.651 &0.660 &0.633 &0.646 &0.716 &0.794 &0.665 &0.737 &0.826 &0.647 &0.709 &0.798 &0.702\\
Liang \emph{et al}.~\cite{liang2022exploring} &0.700 &0.706 &0.829 &0.707 &0.699 &0.794 &0.705 &0.698 &0.844 &0.709 &0.713 &0.851 &0.667 &0.672 &0.750 &0.736\\
CORE~\cite{ni2022core}& 0.658 & 0.708 & 0.917 & 0.630 & 0.644 & 0.807 & 0.671 & 0.708 & 0.923 & 0.663 & 0.711 & 0.925 & 0.653 & 0.689 & 0.920 & 0.748 \\
RECCE~\cite{cao2022end} & 0.635 & 0.756 & \underline{0.933} & 0.636 & 0.604 & 0.821 & 0.661 & 0.724 & \textbf{0.930} & 0.651 & 0.778 & \underline{0.928} & 0.659 & 0.754 & 0.932 & 0.760 \\
FWA~\cite{li2018exposing} & 0.650 & 0.755 & 0.870 & 0.635 & \textbf{0.771} & \underline{0.885} & 0.701 & 0.778 & 0.924 & 0.689 & 0.752 & 0.850 & 0.670 & 0.744 & 0.875 & 0.770 \\
Face X-ray~\cite{li2020face} &0.710 &0.740 &0.890 &0.726 &0.668 &0.838 &0.734 &0.716 &0.899 &0.705 &0.693 &0.907 &0.731 &0.731 &0.901 &0.773\\
SLADD~\cite{chen2022self} & 0.751 & 0.753 & 0.900 & 0.738 & 0.705 & 0.841 & 0.757 & 0.754 & 0.815 & \underline{0.713} & 0.733 & 0.883 & 0.754 & 0.741 & 0.894 & 0.782 \\
F3Net~\cite{qian2020thinking} &0.743 &0.668 &0.926 &0.748 &0.648 &0.872 &\textbf{0.765} &0.692 &0.914 &\textbf{0.719} &0.680 &0.925 &0.779 &0.760 &\underline{0.933} &0.785\\
SRM~\cite{luo2021generalizing} &\underline{0.771} &0.770 &0.915 &0.743 &0.746 &0.874 &0.745 &0.757 &0.909 &0.699 &0.768 &0.923 &0.778 &0.779 &0.891 &0.805\\
SPSL~\cite{liu2021spatial} & 0.742 & \underline{0.787} & 0.927 & \underline{0.749} & \underline{0.753} & \textbf{0.898} & \underline{0.759} & \textbf{0.797} & \underline{0.929} & 0.664 & \underline{0.794} & 0.924  & \underline{0.797} & \textbf{0.813} & 0.924 & \underline{0.817} \\

\midrule

Ours &\textbf{0.805} &\textbf{0.824} &\textbf{0.945} &\textbf{0.767} &0.749 &0.870 &\textbf{0.765} &\underline{0.782} &0.908 &0.711 &\textbf{0.800} &\textbf{0.943} &\textbf{0.800} &\underline{0.808} &\textbf{0.943} &\textbf{0.828}\\
\bottomrule
\end{tabular}}
\vspace{0.1 cm}
\caption{Comparisons of generalization ability with competing methods implemented by ourselves. We use two different data configurations: ``FF-ALL", which includes all data generated by four forgeries, and ``FF-wo-DF", ``FF-wo-F2F", ``FF-wo-FS", and ``FF-wo-NT", which use the FF++ dataset but drop DF, F2F, FS, and NT, respectively. The best results are highlighted in bold font, while the second-best results are underlined.}
\label{tab result}
\vspace{-0.3 cm}
\end{table*}


==> tables/supp_ablation_WD.tex <==
\begin{table*}
  \centering
  \scalebox{0.7}{
  \begin{tabular}{c|c|c|c|c|c|c} \toprule
    \multirow{2}*{Ablation} & DFD & CelebDF-v1 & CelebDF-v2 & DFDCP & DFDC & Avg.\\ 
    \cmidrule(lr){2-2}
    \cmidrule(lr){3-3}
    \cmidrule(lr){4-4}
    \cmidrule(lr){5-5}
    \cmidrule(lr){6-6}
    \cmidrule(lr){7-7}
    & AUC~$\uparrow$ ~\textbar~ AP~$\uparrow$ ~\textbar~ EER~$\downarrow$ & AUC~$\uparrow$ ~\textbar~ AP~$\uparrow$ ~\textbar~ EER~$\downarrow$ & AUC~$\uparrow$ ~\textbar~ AP~$\uparrow$ ~\textbar~ EER~$\downarrow$ & AUC~$\uparrow$ ~\textbar~ AP~$\uparrow$ ~\textbar~ EER~$\downarrow$ & AUC~$\uparrow$ ~\textbar~ AP~$\uparrow$ ~\textbar~ EER~$\downarrow$ & AUC~$\uparrow$ ~\textbar~ AP~$\uparrow$ ~\textbar~ EER~$\downarrow$ \\
    \midrule
    wo AdT & \textbf{0.884} ~\textbar~ \textbf{0.985} ~\textbar~ \textbf{19.8} & 0.860 ~\textbar~ 0.907 ~\textbar~ \textbf{21.7} & 0.824 ~\textbar~ 0.893 ~\textbar~ \textbf{25.7} & 0.800 ~\textbar~ 0.890 ~\textbar~ 27.3 & 0.740 ~\textbar~ \textbf{0.764} ~\textbar~ 32.7 & 0.814 ~\textbar~ 0.888 ~\textbar~ \textbf{25.4} \\
    wo AFT & 0.869 ~\textbar~ 0.982 ~\textbar~ 21.4 & 0.847 ~\textbar~ 0.904 ~\textbar~ 22.1 & 0.809 ~\textbar~ 0.884 ~\textbar~ 26.6 & \textbf{0.815} ~\textbar~ \textbf{0.898} ~\textbar~ \textbf{26.2} & \textbf{0.744} ~\textbar~ 0.762 ~\textbar~ \textbf{32.6} & 0.817 ~\textbar~ 0.886 ~\textbar~ 25.8 \\
    wo CT & 0.881 ~\textbar~ 0.984 ~\textbar~ 19.9 & 0.847 ~\textbar~ 0.898 ~\textbar~ 23.1 & 0.793 ~\textbar~ 0.877 ~\textbar~ 28.4 & 0.793 ~\textbar~ 0.878 ~\textbar~ 28.0 & 0.734 ~\textbar~ 0.756 ~\textbar~ 33.5 & 0.810 ~\textbar~ 0.879 ~\textbar~ 26.6 \\
    \midrule
    Ours & 0.880 ~\textbar~ 0.984 ~\textbar~ 20.0 & \textbf{0.867} ~\textbar~ \textbf{0.922} ~\textbar~ 21.9 & \textbf{0.830} ~\textbar~ \textbf{0.904} ~\textbar~ 25.9 & \textbf{0.815} ~\textbar~ 0.893 ~\textbar~ 26.9 & 0.736 ~\textbar~ 0.760 ~\textbar~ 33.0 & \textbf{0.825} ~\textbar~ \textbf{0.893} ~\textbar~ 25.5 \\
    \bottomrule
  \end{tabular}
  }
  \caption{
  Detailed performance metrics of different ablation studies. The values represent AUC, AP, and EER for each method across various datasets. The average performance (Avg.) across all datasets is also reported. The best results are highlighted in bold.
  }
  \label{tab:ablation_WD}
\end{table*}


==> tables/supp_other_choice_forgery_TS.tex <==
\begin{table*}
  \centering
  \scalebox{0.65}{
  \begin{tabular}{c|c|c|c|c|c|c} \toprule
    \multirow{2}*{Encoder Architecture} & DFD & CDF-v1 & CDF-v2 & DFDCP & DFDC & Avg.\\ 
    \cmidrule(lr){2-2}
    \cmidrule(lr){3-3}
    \cmidrule(lr){4-4}
    \cmidrule(lr){5-5}
    \cmidrule(lr){6-6}
    \cmidrule(lr){7-7}
    & AUC~$\uparrow$ ~\textbar~ AP~$\uparrow$ ~\textbar~ EER~$\downarrow$ & AUC~$\uparrow$ ~\textbar~ AP~$\uparrow$ ~\textbar~ EER~$\downarrow$ & AUC~$\uparrow$ ~\textbar~ AP~$\uparrow$ ~\textbar~ EER~$\downarrow$ & AUC~$\uparrow$ ~\textbar~ AP~$\uparrow$ ~\textbar~ EER~$\downarrow$ & AUC~$\uparrow$ ~\textbar~ AP~$\uparrow$ ~\textbar~ EER~$\downarrow$ & AUC~$\uparrow$ ~\textbar~ AP~$\uparrow$ ~\textbar~ EER~$\downarrow$ \\
    \midrule
    Xception & \textbf{0.888} ~\textbar~ \textbf{0.986} ~\textbar~ 20.3 & 0.823 ~\textbar~ 0.884 ~\textbar~ 23.5 & 0.806 ~\textbar~ 0.882   ~\textbar~ 27.1 & 0.796   ~\textbar~ 0.887 ~\textbar~ 28.5 & 0.729 ~\textbar~ 0.752 ~\textbar~ 34.0 & 0.808 ~\textbar~ 0.878 ~\textbar~ 26.7 \\
    
    EfficientNet-B1 & 0.870 ~\textbar~ 0.983 ~\textbar~ 21.4 & 0.821 ~\textbar~ 0.885 ~\textbar~ 25.1 & 0.809 ~\textbar~ 0.882 ~\textbar~ 27.2 & 0.789 ~\textbar~ 0.881 ~\textbar~ 28.6 & 0.733 ~\textbar~ 0.756 ~\textbar~ 33.5 & 0.804 ~\textbar~ 0.877 ~\textbar~ 27.2 \\

    EfficientNet-B4 & 0.880 ~\textbar~ 0.984 ~\textbar~ \textbf{20.0} & \textbf{0.867} ~\textbar~ \textbf{0.922} ~\textbar~ \textbf{21.9} & 0.830 ~\textbar~ \textbf{0.904} ~\textbar~ \textbf{25.9} & \textbf{0.815} ~\textbar~ \textbf{0.893} ~\textbar~ \textbf{26.9} & 0.736 ~\textbar~ 0.760 ~\textbar~ \textbf{33.0} & \textbf{0.825} ~\textbar~ \textbf{0.893} ~\textbar~ \textbf{25.5} \\
    
    EfficientNet-B5 & 0.877 ~\textbar~ 0.984 ~\textbar~ 21.0 & 0.848 ~\textbar~ 0.919 ~\textbar~ 22.0 & \textbf{0.833} ~\textbar~ 0.898 ~\textbar~ 25.7 & 0.812 ~\textbar~ 0.892 ~\textbar~ 27.1 & \textbf{0.748} ~\textbar~ \textbf{0.772} ~\textbar~ 32.4 & 0.824 ~\textbar~ \textbf{0.893} ~\textbar~ 25.6 \\
    
    \bottomrule
  \end{tabular}
  }
  \caption{
  Performance evaluation of different encoder architectures. All models are trained on the FF++\_c23 dataset and evaluated across various other datasets with metrics presented in the order of AUC~\textbar~AP~\textbar~EER (the frame-level). The average performance (Avg.) across all datasets is also reported. The best results are highlighted in bold.
  }
  \label{tab:other-choice-backbone}
\end{table*}

==> tables/supp_within_entire_synthesis.tex <==
\begin{table}[tb!]
  \centering
%   \vspace{1mm}
  \scalebox{0.75}{
  \begin{tabular}{c|c|c|c|c}
    \toprule
    \multirow{2}*{Method}
    &\multicolumn{4}{c}{Testing Datasets}\\
    \cmidrule(lr){2-5}
    & StarGAN~\cite{choi2018stargan} & DDPM~\cite{ho2020denoising} & DDIM~\cite{song2020denoising} & SD~\cite{rombach2022high} \\
    \midrule
    
    SBI~\cite{shiohara2022detecting} & 0.787 & 0.744 & 0.648 & 0.478 \\

    \midrule

    Ours & \textbf{0.810} &  \textbf{0.854}& \textbf{0.748} & \textbf{0.506} \\
     \bottomrule
  \end{tabular}}
  \caption{
  Results in detecting GAN-generated images and Diffusion-generated images. We compare our results with other augmentation-based SBI~\cite{shiohara2022detecting}. We utilize its official code for evaluation. These models are trained on FF++\_c23. The metric used is the frame-level AUC. ``SD" is the short for stable diffusion.
  }
  \vspace{-10pt}
  \label{tab:ablation_within_entire_synthesis}
\end{table}

